Factorized Inverse Path Tracing for Efficient and Accurate Material-Lighting Estimation

Inverse path tracing has recently been applied to joint material and lighting estimation, given geometry and multi-view HDR observations of an indoor scene. However, it has two major limitations: path tracing is expensive to compute, and ambiguities exist between reflection and emission. Our Factorized Inverse Path Tracing (FIPT) addresses these challenges by using a factored light transport formulation and finds emitters driven by rendering errors. Our algorithm enables accurate material and lighting optimization faster than previous work, and is more effective at resolving ambiguities. The exhaustive experiments on synthetic scenes show that our method (1) outperforms state-of-the-art indoor inverse rendering and relighting methods particularly in the presence of complex illumination effects; (2) speeds up inverse path tracing optimization to less than an hour. We further demonstrate robustness to noisy inputs through material and lighting estimates that allow plausible relighting in a real scene. The source code is available at: https://github.com/lwwu2/fipt

==> equations/emission-loss.tex <==
\begin{equation}
    l_e=\lambda_e\sum_\mathbf{x}\Vert\text{MLP}_\text{emit}(\mathbf{x})\Vert_1,\lambda_e=1.
    \label{eq:emission-loss}
\end{equation}

==> equations/emission-network.tex <==
\begin{equation}
    \alpha=1-\exp{
    \left(-\max(\text{MLP}_\text{emit}(\mathbf{x}),0)\right)
    }
\end{equation}

==> equations/incident-light.tex <==
\begin{equation}
    \mathbf{L}_i(\bm{\omega}_i)=
    \mathbf{L}(\text{rayIntersect}(\mathbf{x},\bm{\omega}_i;\text{scene}),-\bm{\omega}_i).
    \label{eq:incident-light}
\end{equation}

==> equations/rendering-equation-no-emit.tex <==
\begin{equation}
    \mathbf{L}_r(\mathbf{x},\bm{\omega}_o)
    = \int_{\Omega^+} \mathbf{L}_i(\mathbf{x},\bm{\omega}_i)
    f(\mathbf{x},\bm{\omega}_i,\bm{\omega}_o)d\bm{\omega}_i,
    \label{eq:rendering-equation-no-emit}
\end{equation}

==> equations/shading-abstract.tex <==
\begin{equation}
\begin{gathered}
    \mathbf{L}_*(\mathbf{x},\bm{\omega}_o)
    = \int_{\Omega^+}\mathbf{L}_i(\mathbf{x},\bm{\omega}_i)g(\mathbf{x},\bm{\omega}_i,\bm{\omega}_o)d\bm{\omega}_i,
    \label{eq:shading-abstract}
\end{gathered}
\end{equation}

==> figures/teaser_new.tex <==
\begin{figure}
    \centering
    % \includegraphics[width=0.99\linewidth]{images/teaser_final_v2.pdf}
    \includegraphics[width=0.99\linewidth]{images/teaser_final_v3.pdf}
    
    \setlength{\tabcolsep}{0.5pt}
    \resizebox{0.99\linewidth}{!}{
        \begin{tabular}{cccc}
             \includegraphics[width=0.3\linewidth]{images/real/real_conference_geometry.png}&
             \includegraphics[width=0.3\linewidth]{images/real/real_conference_albedo.png}&
             \includegraphics[width=0.3\linewidth]{images/real/real_conference_roughness.png}&
             \includegraphics[width=0.3\linewidth]{images/real/real_conference_emission.png}\\[-0.7ex]
             Geometry (Est.) & $\mathbf{a}'$ & Roughness & Emission\\[-0.25ex]
             \includegraphics[width=0.3\linewidth]{images/real/real_conference_rgb.png}&
             \includegraphics[width=0.3\linewidth]{images/real/real_conference_rerender.png}&
             \includegraphics[width=0.3\linewidth]{images/real/real_conference_render.png}&
             \includegraphics[width=0.3\linewidth]{images/real/real_conference_relight.png}
             \\[-0.7ex]
            RGB input & Rendered & View synthesis & Relight 
        \end{tabular}
    }
    
    \caption{
    \textbf{Ours vs. baselines.} 
        (Upper) \ipt~takes a piecewise constant parameterization of material to reduce Monte Carlo variance and ambiguity for inverse rendering,
        losing fine spatial details as a result. 
        Directly extending it to complex material representation (\eg\milo) shows very slow convergence.
        In contrast,
        we propose Factorized Inverse Path Tracing (FIPT) to get rid of variance and reduce ambiguities,
        yielding efficient and high quality BRDF-emission (4th row),
        appealing relighting (1st row), and object insertion (the bunny on the table).
        The presented scene is synthetic with the inset showing the input (lower-left sub-figure).
        (Lower) 
    }
    \label{fig:teaser}
\end{figure}



==> tables/synthetic-brdf-avg.tex <==
\begin{table}[t]
    \centering
    \setlength\tabcolsep{3.0pt}
    \resizebox{0.99\linewidth}{!}{
\begin{tabular}{clccccc}
\toprule
%ours ours-sem lieccv22 neilf milo
& \multirow{2}{*}{Method} & 
$\mathbf{k}_d$ & $\mathbf{a}'$ & $\sigma$ &
\multicolumn{2}{c}{$\mathbf{L}_e$} \\
&
&\multicolumn{3}{c}{PSNR$\uparrow$} & 
IoU$\uparrow$ & logL2$\downarrow$\\
\midrule
\multirow{5}{*}{Bathroom} &
\lieccv & 19.92 & 15.78 & 13.77 & 0.45 & 1.35\\
&\neilf & 10.12 & 9.01 & 14.82 & - & - \\
& \ipt & 22.43 & 18.59 & 14.69 & 0.33 & 1.09e-1\\
&\milo & 11.68 & 9.29 & 5.02 & 0.05 & 4.90e-1\\
&\ours & \textbf{30.13} & \textbf{25.28} & \textbf{28.79} & \textbf{0.63} & \textbf{3.18e-2}\\
&\ours-sem & 27.81 & 24.00 & 21.84 & \textbf{0.63} & \textbf{3.18e-2}\\

\midrule
\multirow{5}{*}{Bedroom} &
\lieccv & 21.87 & 17.18 & 12.12 & 0.34 & 2.78\\
&\neilf & 14.88 & 12.42 & 11.30 & - & - \\
& \ipt & 29.39 & 22.46 & 13.33 & 0.92 & 4.01e-3\\
&\milo & 18.65 & 14.99 & 6.38 & 0.08 & 1.60e-2\\
&\ours & \textbf{31.10} & \textbf{29.41} & 23.19 & \textbf{0.96} & 4.95e-4\\
&\ours-sem & 31.00 & 28.45 & \textbf{25.23} & \textbf{0.96} & \textbf{4.93e-4}\\

\midrule
\multirow{5}{*}{Livingroom} &
\lieccv & 17.25 & 15.32 & 12.72 & 0.17 & 3.61\\
&\neilf & 12.34 & 10.97 & 13.45 & - & - \\
& \ipt & 21.24 & 19.01 & 11.77 & 0.90 & 6.08e-3\\
&\milo & 18.52 & 15.73 & 6.06 & 0.06 & 1.93e-2\\
&\ours & 28.86 & \textbf{28.70} & \textbf{32.48} & \textbf{0.95} & \textbf{8.06e-4}\\
&\ours-sem & \textbf{29.09} & 28.62 & 25.15 & \textbf{0.95} & 8.09e-4\\

\midrule
\multirow{5}{*}{Kitchen} &
\lieccv & 18.14 & 14.54 & 10.82 & 0.43 & 1.41\\
&\neilf & 12.63 & 9.96 & 10.64 & - & - \\
&\ipt & 25.68 & 21.61 & 11.84 & 0.83 & 1.08e-2\\
&\milo & 15.69 & 11.48 & 8.39 & 0.10 & 1.86e-1\\
&\ours & 33.07 & \textbf{27.53} & \textbf{29.24} & \textbf{0.91} & \textbf{1.54e-3}\\
&\ours-sem & \textbf{33.25} & 27.38 & 21.70 & \textbf{0.91} & \textbf{1.54e-3}\\
\bottomrule
\end{tabular}
}
    \caption{\textbf{BRDF-emission comparison on synthetic scenes} 
    shows that our method gives the overall best reconstruction.
    The results are similar even if only semantic segmentation is provided (\ours-sem).
    NeILF does not estimate emitters. The best method is marked in bold.
    }
    \label{tab:synthetic-brdf}
\end{table}
